GitHub-OSS Fixit: Fixing bugs at scale in a Software Engineering Course

Many studies have shown the benefits of introducing open-source projects into teaching Software Engineering (SE) courses. However, there are several limitations of existing studies that limit the wide adaptation of open-source projects in a classroom setting, including (1) the selected project is limited to one particular project, (2) most studies only investigated on its effect on teaching a specific SE concept, and (3) students may make mistakes in their contribution which leads to poor quality code. Meanwhile, software companies have successfully launched programs like Google Summer of Code (GSoC) and FindBugs "fixit" to contribute to open-source projects. Inspired by the success of these programs, we propose GitHub-OSS Fixit, a course project where students are taught to contribute to open-source Java projects by fixing bugs reported in GitHub. We described our course outline to teach students SE concepts by encouraging the usages of several automated program analysis tools. We also included the carefully designed instructions that we gave to students for participating in GitHub-OSS Fixit. As all lectures and labs are conducted online, we think that our course design could help in guiding future online SE courses. Overall, our survey results show that students think that GitHub-OSS Fixit could help them to improve many skills and apply the knowledge taught in class. In total, 154 students have submitted 214 pull requests to 24 different Java projects, in which 59 of them have been merged, and 82 have been closed by developers.

==> Makefile <==
all:
	#gnuplot run-gnuplot
	#\put(3875,1188){\rotatebox{60}{\makebox(0,0)[r]{\strut{}\shortstack{Not\\{} reproducible}}}}%
	pdflatex main.tex
	bibtex main
	pdflatex main.tex
	pdflatex main.tex
	dvips -Ppdf -G0 -t a4 main.dvi
	pdftops main.pdf
	#ps2pdf -dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true -dPDFSETTINGS=/prepress main.pdf main-output.pdf
	ps2pdf -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress main.ps main.pdf
	pdftk A=main-output.pdf cat A1-end output nobookmarks.pdf
.PHONY:clean
clean:
	\rm *.aux *.blg *.bbl *.log


==> implementation.tex <==
\subsection{Implementation}
For calculating code similarity, we leverage JPlag~\cite{prechelt2002finding}. JPlag compares two sets of programs by trying to cover one of the programs with sequences from the other program using the maximum similarity algorithm~\footnote{https://jplag.ipd.kit.edu/example/help-sim-en.html}. While there are many code plagiarism detection engines that can calculate code similarity~\cite{prechelt2002finding,ahtiainen2006plaggie,luo2014semantics,martins2014plagiarism,lancaster2004comparison,schleimer2003winnowing}, we select JPlag because (1) it is open-source and actively maintained, (2) it offers offline similarity analysis, and (3) it has been shown to be one of the most effective code similarity analyzers~\cite{ragkhitwetsagul2018comparison,7522248}. To compute the dependency similarity, we support projects that use Gradle~\footnote{https://gradle.org/} and Maven~\footnote{https://maven.apache.org/} for compilations because (1) they are among the most popular open source build automation tools, and (2) Gradle has been widely used in both Java and Android projects. We compute UI similarity by modifying existing implementation of Bugine, a tool that recommends relevant GitHub issues based on UI similarity~\cite{collabbug}. The main modification to Bugine is to add the support for incorporating the open GitHub issue $d$ into the UI similarity calculation.


==> knowledge.tex <==
\begin{table*}[t]
\small
\centering
\caption{Survey results for the question ``During the \mytool{}, I have improved my skills on:''}
  \label{tab:knowledge}
\begin{tabular}{l|r|r|r|r|r|}
Knowledge                                & Strongly Disagree & Disagree   & Neutral     & Agree       & Strong Agree \\\hline
Version Control System (Git):            & 3(2.13\%)       & 1(0.71\%)  & 11(7.8\%)   & \textbf{71(50.35\%)} & 55(39.01\%)          \\
GitHub (read issues, make pull requests): & 3(2.13\%)       & 1(0.71\%)  & 6(4.26\%)   & 60(42.55\%)          & \textbf{71(50.35\%)} \\
Unit test (JUnit):                       & 3(2.13\%)       & 1(0.71\%)  & 8(5.67\%)   & \textbf{69(48.94\%)} & 60(42.55\%)          \\
System/Integration tests (non JUnit):    & 5(3.55\%)       & 10(7.09\%) & 46(32.62\%) & \textbf{51(36.17\%)} & 29(20.57\%)          \\
Code comment (Javadoc):                  & 3(2.13\%)       & 3(2.13\%)  & 16(11.35\%) & \textbf{70(49.65\%)} & 49(34.75\%)          \\
Coding standard:                         & 4(2.84\%)       & 0(0\%)     & 21(14.89\%) & \textbf{63(44.68\%)} & 53(37.59\%)          \\
Test-driven development (TDD):           & 4(2.84\%)       & 6(4.26\%)  & 38(26.95\%) & \textbf{58(41.13\%)} & 35(24.82\%)          \\
Knowledge about Java programming         & 4(2.84\%)       & 2(1.42\%)  & 20(14.18\%) & \textbf{73(51.77\%)} & 42(29.79\%)          \\
Static Analysis Tools:                   & 3(2.13\%)       & 1(0.71\%)  & 12(8.51\%)  & 60(42.55\%)          & \textbf{65(46.1\%)}  \\
Working in a team:                       & 3(2.13\%)       & 8(5.67\%)  & 21(14.89\%) & \textbf{62(43.97\%)} & 47(33.33\%)   
\end{tabular}
\end{table*}


==> mystudy.tex <==
%\section{Motivation}
%Although Android apps are typically developed using Java programming language, they are different from traditional desktop applications and server applications. Particularly, Android applications rely heavily on a set of software components (e.g., Activity, Intent and Content Service Provider) supported by the Android Development framework with specific rules for managing these components~\footnote{http://developer.android.com/guide/}.
%
%%Crashes in Android applications arise due to several reasons, including (1) Android-specific bugs that occurs due to the complexity in Android activity lifecycle~\cite{hu2011automating,coelho2016exception}, and (2) programming mistakes that are also common sources of errors in Java development~\cite{coelho2016exception}. Meanwhile, prior work on automated testing and analysis~\cite{hu2011automating,coelho2016exception}
%%Despite the prevalence of crashes due to the complexity of Android activity lifecycle.
%
%Prior works on Android applications reveal that the complexity in Android activity lifecycle is one of the major causes of crashes in Android applications~\cite{hu2011automating,coelho2016exception}. Despite recent advances in automated testing and analysis of Android applications, there is no existing work that suggest patches to crashes in Android applications.

\section{A study of similar bugs in GitHub}
\label{sec:study-cause}
Given an open and unresolved GitHub issues $d$, identifying a relevant GitHub issues $n$ that shares similar bug with $d$ could be useful for localizing and fixing the bug in $n$. To design more effective tools to search for relevant GitHub issues, we need to first thoroughly understand the characteristics of similar bugs, including answering the research questions (\textbf{RQ1}-\textbf{RQ3}) listed in Section~\ref{sec:intro}. We investigate $RQ1$ because prior study shows that similar bugs could exist among two different applications~\cite{collabbug} but the precise definition and the characteristics of ``similar bugs'' have not been investigated. We study $RQ2$ to design better tools to better utilize and extract information from GitHub issues with similar bugs. We design $RQ3$ to investigate the usefulness of referring to GitHub issues with similar bugs.

\input{study-table}

%\begin{description}[leftmargin=*]
%        \item[RQ1:] \emph{What are the common characteristics that define similar bugs?} What are the exact similarities in the related GitHub issues that developers refer to as ``similar bugs''?
%        %\item[Q2:] \emph{How often do developers refer to similar bugs in another repositories?} Specifically, what percentages of similar bugs are from two GitHub issues of different repositories?
%        \item[RQ2:] \emph{What strategies can we use to identify the pair of similar issues?} Can we derive a set of strategies to automatically identify these similar issues?
%        \item[RQ3:] \emph{How do developers make use of information about similar bugs?} Specifically, which software maintenance tasks that the similar bugs could assist developer with, if any? 
%\end{description}

%Same co(Android/Window version, Device, Permission set)

%We investigate $Q2$ to identify strategies that can be used to automatically search for issues with similar bugs.We study $Q2$ to investigate the prevalence of similar bugs found across different software project~\cite{collabbug}. 


To study the relationship between GitHub issues that share similar bug, we manually inspected related GitHub issues. Our goal is to identify the information that we can obtain from GitHub issues with similar bugs. We first obtained a list of GitHub issues by searching for the keywords ``similar bug'' and ``similar problem'' written in Java using \texttt{PyGitHub} (a Python library that interacts with GitHub API v3)~\footnote{https://github.com/PyGithub/PyGithub}. Our study focuses on Java projects because (1) most of the recent automated program repair techniques have been developed for fixing Java programs~\cite{xiong2017precise,jiang2018shaping,mei-et-al-ASE15,wen2018context,liu2019tbar} (including the recent bug report driven repair approach~\cite{bugreportrepair}), which indicates the importance of building an automated program repair system for Java programs; and (2) prior work on \cofind{} shows the existence of similar bugs across different Android apps while most Android apps are written in Java. For each issue $d$, our crawler searched for the first corresponding issue $n$ in which $d$ mentioned that $d$ and $n$ share similar bugs. The final output of our crawler is a list of GitHub issues ($d$, $n$) where $d$ and $n$ share similar bugs. Overall, our crawler searched through 4000 GitHub issues (GitHub API limits each search to 1000 search results~\footnote{https://docs.github.com/en/rest/reference/search}, so we search for the two keywords with 1000 open and 1000 closed issues separately), and identified 385 issues with links to similar bugs. From these 385 GitHub issues, we manually excluded 194 invalid issues (e.g., duplicated issues or irrelevant issues). After filtering the irrelevant issues, we identified \numstudy{} ($n$, $d$) pairs of GitHub issues where $n$ spans across \numstudyproj{} different Java projects. This relatively large number of open-source projects with GitHub issues mentioning similar bugs confirm with our hypothesis that \emph{software developers tend to leverage the information about similar bugs during the discussion of a GitHub issue}.

 %We manually analyzed all issues and attempted to answer two questions:

% Overall, our crawler searched through 4000 GitHub issues (\texttt{PyGitHub} limits each search to 1000 search results so we search for the two keywords with 1000 open and 1000 closed issues separately). From the original list of GitHub issues, we manually removed issues that do not have corresponding issues with similar bugs. After filtering the irrelevant issues, we identified \numstudy{} ($i$, $j$) pairs of GitHub issues that span across \numstudyproj{} different Java projects. %We manually analyzed all issues and attempted to answer two questions:

\subsection{RQ1: Characteristic of similar bugs}
For RQ1, we obtain the characteristic of similar bugs by reading carefully the GitHub issues, focusing particularly on comments made by developers when referring to the similar bugs (i.e., developers usually include explanation why the two bugs are similar). Then, we count the number of GitHub issues that exhibit the identified characteristics. 

The second column of Table~\ref{tab:study-tab} shows the common characteristics that define similar bugs in the evaluated pairs of GitHub issues, whereas the ``\# of Issues'' column denotes the number of GitHub issues that exhibit these characteristics. Our study shows that similar bugs can be defined by bugs that occur when two GitHub projects share the (1) same libraries, (2) same functionality, (3) same steps to reproduce, (4) same configuration/environment, (5) same outcome (exclude crash), or (6) same error/exception. As a pair of GitHub issues ($d$, $n$) can exhibit several similarities (e.g., they could share same libraries and produce the same error as the example in Table~\ref{tab:similar-bug}), we include all similarities in Table~\ref{tab:study-tab} (the category is mutually exclusive). Overall, our study shows that the most common characteristics of similar bugs are:
\begin{itemize}
\item Bugs that share the same library (76/\numstudy{} = 50\%)  
\item Bugs that share the same error/exception (39/\numstudy{} = 26\%)%26\%)
\item Bugs that share the same outcome (35/\numstudy{} = 23.33\%) %26\%)
\end{itemize}

The relatively high percentage of bugs that share the same library \emph{motivates the needs for automated dependency update tools}~\cite{dependabot,greenkeeper,macho2018automatically}.

\subsection{RQ2: Strategies to identify similar bugs}
\label{subsec:rqtwo}
After identifying the common characteristics of similar bugs, we need to design strategies to automatically detect these characteristics. Specifically, we need to check if we can detect each of these characteristics from several available sources, including: (1) the description of a GitHub issue, and (2) information within different types of files that can be exploited for detecting these characteristics (e.g., Java projects typically has build files and Java class files, whereas Android project may have additional XML files for declaring app components and permissions). 

Given a pair of GitHub issues ($d$, $n$) that share a similar bug $b$, we derive \numop{} strategies to identify similar bugs based on the rules explained below:

\begin{description}[leftmargin=*]
\item[Dependency:] We check if $d$ and $n$ share the same libraries by comparing the set of dependencies shared by the GitHub issues in $d$ and $n$. For example, in Table~\ref{tab:similar-bug}, both \texttt{Maui} and \texttt{deeplearning4j} share similar dependency (Stemmer library). The dependencies of Java projects are usually declared in their build files. 
\item[Code:] We check if $d$ and $n$ share similar functionalities by comparing the Java code in the repository for $d$ and the code modifications in the patch mentioned in $n$. 
\item[UI (Android-specific):] We check if $d$ and $n$ share the same steps to reproduce the bug $b$ by comparing their interfaces that allow users to invoke these steps. In Android apps, interfaces refer to UI elements (e.g., buttons and text boxes) that are typically declared in XML files.
\item[Permission (Android-specific):] We check if $d$ and $n$ share similar environments by comparing the set of permissions that $d$ and $n$ acquire. We design this Android-specific strategy as all Android apps are required to declare the set of permissions in their manifest files but there is no such formal requirement for other Java projects. The set of permissions for Android apps is typically declared in XML files. 
\item[Condition:] We can check if $d$ and $n$ share the same outcomes by comparing the conditions before the bug $b$ is triggered. This information is usually available in the description of a GitHub issue.  
\item[Stack trace:] We can check if $d$ and $n$ share the same error or exception by comparing their stack traces. For example, in Table~\ref{tab:similar-bug}, the issues in \texttt{Maui} and \texttt{deeplearning4j} share similar stack trace with similar exception. This information is usually available in the description of a GitHub issue.   
\end{description} 


 \begin{figure}
    \begin{minipage}[t]{\linewidth}
        \centering
        %\includegraphics[height=3.5cm,width=0.41\linewidth]{How_can_issues_help_4classes.png}
        \includegraphics[height=4.4cm]{How_can_issues_help_4classes.eps}
    \caption{The usefulness of similar bugs}
\label{fig:usefulness}
    \end{minipage}
\end{figure}
\subsection{RQ3: Usefulness of similar bugs}
We investigate the usefulness of similar bugs by checking whether the \numstudy{} issues help developers to perform specific maintenance tasks by scoring them in the following order: (1) repair (most useful), (2) fault localization, (3) finding context of a bug, and (4) closing the issue faster (least useful). Specifically, if the similar bug could help developer directly in locating and fixing the bug, we select the most useful task (``repair'') rather than ``fault localization''. During our analysis, we exclude 64 GitHub issues from \numstudy{} because we could not determine their usefulness as there are no direct reply or discussion about the similar issue.

Given a pair of GitHub issues ($d$, $n$), we assess $n$'s usefulness based on the rationale explained below:
\begin{description}[leftmargin=*]
\item[Repair:] We consider $n$ as helping developer in $d$ to repair the bug in $d$ if: (1) the fix of $n$ could be directly applied to $d$, (2) the fix of $n$ only requires minor modifications before applying to $d$, or (3) the discussion of $d$ mentioned that they could find the fix for $d$ by referring to the information in $n$.
\item[Fault localization:] We consider $n$ as helping developer in $d$ to locate the bug if: (1) $n$ causes the bug in $d$, (2) $n$ includes fault localization information, or (3) the discussion of $d$ mentioned that they could identify the faulty location using the information in $n$. 
\item[Context:] We consider $n$ as helping developer in $d$ to finding more context for the bug in $d$ if the discussion in $d$ explicitly mentioned that they have learned something from $n$ (e.g., they gained some clues after reading $n$) but there is no further discussion about whether the knowledge gained had helped them in resolving the problem or identifying the fault. 
\item[Closing Issue faster:] We consider $n$ as helping developer in $d$ to closing the issue faster if: (1) after referring to the similar issue in $n$, the participants in the discussion of $d$ think that they cannot or do not need to fix the bug and decided to close the issue, or (2) $n$ only provides temporary workaround.
\end{description}

Figure~\ref{fig:usefulness} shows the usefulness of similar bugs among the 86 studied issues. Our study shows that similar bugs is most helpful in terms of helping developers to find more context (provide hints) for resolving the bug (\studycontext{} of studied GitHub issues). Meanwhile, \studyrepair{} of studied issues show the usefulness of similar bugs in helping developers to fix the bug. Overall, our results shows that \emph{similar bugs could help developers in resolving the GitHub issue in hand, especially in providing more context of the bug and fixing the bug}.

%situations of repair: 
%1. the fix of the referred issue totally applies to current issue
%2. the fix of the referred issue only requires minor modification to apply to current issue
%3. the participant found out fixes with the help of info in referred issues


%situations of fault localization: (however, if there is no further discussion about fix or workaround, we cannot decide if the participant identifies fault correctly, thus, in most times, I will classify them as context)
%1. the referred issue is the cause of current issue
%2. there is fault identification info in the referred issue
%3. the participant identified faults with the help of info in referred issues 

%situations of context:
%1. the author or other participants learned something from the referred issue, e.g., they had some clues, guess, or ideas inspired by the referred issue and explicitly state them as comments. However, no commends afterwards verify that the ideas successfully solve the problem or identify the fault. 

%situations of closing faster:
%1. after referring to the similar issue, participants think they cannot/don’t need to/ fix the bug and close the issue.
%2. the referred issue provides applicable temporary workaround
 
%Table~\ref{tab:exception} shows the set of exceptions that lead to crashes in the investigated Android apps and the percentage of GitHub issues that arise due to particular exception. Table~\ref{tab:exception} illustrates that 
%The high percentage of \texttt{NullPointerException} confirms with the findings of prior study of Android apps~\cite{coelho2016exception}. 

%Note that the ``Unknown" row represents the scenario where the bug report did not include the information about the thrown exception. Although there are many such cases, this does not pose threat to our investigation as we could still derive the root cause of the crash through inspection of the bug-fixing commit.

%Table~\ref{tab:study-tab} shows the common root causes of crashes in Android apps we investigated. Column ``Category" in Table~\ref{tab:rootcause} describes the high-level causes of the crashes, while the ``Specific reasons" column gives the specific causes that lead to the crash. The last column (Category Total (\%)) presents the total percentage of issues that fits into a particular category. Overall, 14.02\% of crashes in our study occur due to the violation of management rules for Android Activity/Fragment lifecycles. The reader can refer to Section~\ref{sec:pattern} on the explanation of these lifecycle-related crashes. Meanwhile, 16.82\% of the investigated crashes are due to improper handling of resources, including resources either not available (Resource-related) or limited resources like memory (Resource limit). Furthermore, improper handling of callbacks contributes to 17.76\% of crashes. Note that this ``Callback" category denotes implementation-specific problems of different components in Android library (e.g., Activity, View and Intent). Among 40.19\% of NullPointerExceptions thrown in these crashing apps, only 12.15\% is related to missing the check for \texttt{null} objects (Missing Null-check). Interestingly, 4.67\% of the GitHub issues include comments by Android developers acknowledging the fact that the patch issued are merely temporary fixes (Workaround) for these crashes that may require future patches to completely resolve the crash.

%Overall, Table~\ref{tab:rootcause} shows that the complexity of activity/fragment lifecycle and incorrect resource handling are two general causes of crashes in Android apps. Moreover, ``Missing Null-check" in the ``Other" category also often leads to crashes in Android apps.



%Regardless what is the reason for introducing these errorsduring bug fixing and why they were not caught before re-lease, their common existences and severe impacts on users and vendors have raised some serious concerns about thebug fixing process. In order to come up with better process and more effective tools to address this problem, we need to first thoroughly understand the characteristics of incorrectfixes, including:

%We study $Q2$ because a survey of Android developers suggests that the topmost reasons (47\%) for \texttt{NullPointerException} in Android apps occur due to the complexity of activity/fragment lifecycle~\cite{coelho2016exception}. Our goal is to identify a set of generic transformations that are often used by Android developers in fixing Android apps. To gain deeper understanding of the root causes of each crash (Q1) and to identify the affect of activity/fragment lifecycle on the likelihood of introducing crashes (Q2), we manually examine lifecycle management rules in the official Android API documentations~\footnote{https://developer.android.com/guide/components/activities/activity-lifecycle.html}. 


%We focus on closed issues because those issues have been confirmed by the developers and are more likely to contain fixes for the crashes. From the list of closed issues on app crashes, we further extract issues that contain at least one corresponding commit associated with the crash. The final output of our crawler is a list of crashes-related closed issues that have been fixed by the developers. Overall, our crawler searches through 7691 GitHub closed issues where 1155 (15\%) of these issues are related to crashes. The relatively high percentage of crash-related issues indicates the prevalence of crashes in Android apps. Among these 1155 issues, 107 of these issues from 15 different apps have corresponding bug-fixing commits. We manually analyzed all issues and attempted to answer two questions:





%To study the root causes of crashes in Android apps, we manually inspect Android apps on GitHub and API documentation (as prior work has showed success in finding bugs via API documentation~\cite{Tan:2012:TTJ:2224481.2224930}). Our goal is to identify a set of common causes for Android crashes. We first obtain a set of popular Android apps by crawling GitHub and searching for the word ``android app'' written in Java using the GitHub API~\footnote{https://developer.github.com/v3/}. For each app repository, we search for closed issues (resolved bug report) with the word ``crash''. We focus on closed issues because those issues have been confirmed by the developers and are more likely to contain fixes for the crashes. From the list of closed issues on app crashes, we further extract issues that contain at least one corresponding commit associated with the crash. The final output of our crawler is a list of crashes-related closed issues that have been fixed by the developers. Overall, our crawler searches through 7691 GitHub closed issues where 1155 (15\%) of these issues are related to crashes. The relatively high percentage of crash-related issues indicates the prevalence of crashes in Android apps. Among these 1155 issues, 107 of these issues from 15 different apps have corresponding bug-fixing commits. We manually analyzed all issues and attempted to answer two questions:
%\begin{description}
%	\item[Q1:] What are the possible root causes and exceptions that lead to crashes in Android apps?
%        \item[Q2:] How does the complexity of activity/fragment lifecycle affect crashes in Android apps? 
%\end{description}

%We study $Q2$ because a survey of Android developers suggests that the topmost reasons (47\%) for \texttt{NullPointerException} in Android apps occur due to the complexity of activity/fragment lifecycle~\cite{coelho2016exception}. Our goal is to identify a set of generic transformations that are often used by Android developers in fixing Android apps. To gain deeper understanding of the root causes of each crash (Q1) and to identify the affect of activity/fragment lifecycle on the likelihood of introducing crashes (Q2), we manually examine lifecycle management rules in the official Android API documentations~\footnote{https://developer.android.com/guide/components/activities/activity-lifecycle.html}. 

%Indeed, the Android API documentation provides detailed explanations about the ``Lifecycle" and ``Resource" category, together with guidelines of the correct handling mechanism for these two categories.
%Therefore, we focus on the ``Lifecycle" category and the ``Resource" category for our derivation of program transformations.


==> online-query-table.tex <==
\begin{table*}[t]
\centering
 \caption{Strategies used in extracting information to build the online query}
\label{tab:online-query}
 \resizebox{\linewidth}{!} {
\setlength\tabcolsep{0.9pt}
\begin{tabular}{c|l|l|l|l}
\multicolumn{1}{c}{Strategy}    & \multicolumn{1}{c}{Description} & \multicolumn{1}{c}{Source} & \multicolumn{1}{c}{Example Text}                                       & \multicolumn{1}{c}{Generated Query} \\ \hline
Stack trace & \begin{tabular}[c]{@{}l@{}}Exception/Error type and \\ exception/error message\\ in the stack trace\end{tabular} & issue body & 
 \begin{tabular}[c]{@{}l@{}}java.lang.\textbf{NullPointerException}: \textbf{Attempt to invoke}\\ \textbf{virtual method} '\textbf{java}.\textbf{lang}.\textbf{Object} \textbf{android}.\textbf{widget}\\.\textbf{FrameLayout}.\textbf{getTag(int)}' \textbf{on a null object reference}\end{tabular} & \begin{tabular}[c]{@{}l@{}}NullPointerException attempt to invoke virtual method \\java lang Object android widget FrameLayout getTag int\\ on a null object reference\end{tabular}\\\hline
Condition & \begin{tabular}[c]{@{}l@{}} Condition where the buggy\\ behavior is triggered\end{tabular} & issue title
   &
 \begin{tabular}[c]{@{}l@{}}  Stemmer exception when \textbf{training word2vec with} \\\textbf{the supplied tweets\_clean.txt file}\end{tabular} &
  training word2vec with the supplied tweets\_clean.txt file \\\hline
Summary &\begin{tabular}[c]{@{}l@{}}summary of the bug from title\end{tabular} & issue title & \textbf{SwedishStemmer} (and \textbf{DutchStemmer}?) not \textbf{thread safe} & SwedishStemmer DutchStemmer thread safe
\end{tabular}}
\end{table*}


==> result-table.tex <==
\begin{table*}[!t]
\small
\caption{Statistics and Evaluation Results of the Android apps used}
  \label{tab:app-stat}
\begin{tabular}{llrrrrrrr}
\hline
\multirow{2}{*}{\textbf{App Name}}   & \multirow{2}{*}{\textbf{Category}} &\multirow{2}{*}{\textbf{KLOC}} & \multirow{2}{*}{\textbf{\#Downloads}} & \multirow{2}{*}{\textbf{Rating}} & \multirow{2}{*}{\textbf{Version No.}} & \textbf{\#GitHub} &  \textbf{\#GitHub Issue} & \textbf{\# Bugs Found} \\
& & & & & &  \textbf{Stars}& \textbf{(closed)} & \textbf{(new,old)} \\ \toprule
Camera-Roll         & Gallery           & 26.00         & 100,000+             & 4.2             & 1.0.6                & 420                    & 227(133)       & (11, 0)                     \\ \hline
PocketHub           & GitHub client     & 31.35         & 10,000+              & 3.3             & 0.5.1                & 9429                   & 644(526)       & (12, 2)                    \\ \hline
Simple File Manager & Explorer          & 5.84          & 50,000+              & 4.5             & 6.3.4                & 378                    & 189(130)       & (6,  2)            \\ \hline
Zapp                & Broadcast         & 8.41          & N.A.                 & N.A.            & 3.2.0                & 60                     & 151(137)       & (2,  7)          \\ \hline
Simpletask          & Reminder          & 24.80         & 10,000+              & 4.7             & 10.3.0               & 349                    & 821(583)       & (3,  2)        \\ \hline
\end{tabular}
\end{table*}


==> second.tex <==
\begin{lstlisting}[language=java,basicstyle=\scriptsize,caption=Our recommended patch for,upquote=true,label={lst:droixpatch2}]
^$\Plus$^ private static Collection<String> split(String value, int charSize) {
^$\Plus$^   List<String> strings = new ArrayList<String>();
^$\Plus$^   int index = 0;
^$\Plus$^   while (index < value.length()) {
^$\Plus$^    strings.add(value.substring(index, Math.min(index + charSize, value.length())));
^$\Plus$^    index += charSize;
^$\Plus$^   }
^$\Plus$^   return strings; }

^$\Minus$^  raf.writeUTF((String) value);
^$\Plus$^  if (isBigString(ad)) {// if attribute descriptor marked as Big String
^$\Plus$^  String strVal = (String) value;
^$\Plus$^  List<String> values = new ArrayList<>();
^$\Plus$^  // if bytes length is over the maximum allowed, calculate parts
^$\Plus$^    if (strVal.getBytes().length >= MAX_BYTES_LENGTH) {
^$\Plus$^     values.addAll(split(strVal, 32767));
^$\Plus$^    } else { values.add(strVal);}

^$\Plus$^     // write total parts
^$\Plus$^     raf.writeInt(values.size());
^$\Plus$^     // write every string chunk
^$\Plus$^     for (String evalue : values){
^$\Plus$^      raf.writeUTF(evalue);
^$\Plus$^     }
^$\Plus$^  } else {// normal string encoding
^$\Plus$^     raf.writeUTF((String) value);
^$\Plus$^  }

^$\Minus$^  return raf.readUTF();
^$\Plus$^   if (isBigString(ad)) {
^$\Plus$^        // read total parts
^$\Plus$^        int parts = raf.readInt();
^$\Plus$^        // read every part
^$\Plus$^        StringBuilder sb = new StringBuilder();
^$\Plus$^        for (int i = 0; i < parts; i++) {
^$\Plus$^            sb.append(raf.readUTF());
^$\Plus$^        }
^$\Plus$^        return sb.toString();
^$\Plus$^    } else {
^$\Plus$^        return raf.readUTF();
^$\Plus$^    }
\end{lstlisting}



==> study-table.tex <==
\begin{table}[t]
\centering
 \caption{Common characteristics of similar bugs, and strategies to identify them (\emph{one issue could have multiple characteristics})}
\label{tab:study-tab}
 \resizebox{\linewidth}{!} {
%\begin{tabular}{|l|l|r|}
\setlength\tabcolsep{0.9pt}
\begin{tabular}{l|l|r}
Strategy  & Characteristic of similar bugs & \# of Issues\\ \hline
Dependency  & Same library                  & 76 \\ \hline%\cline{2-3}%75\hline
Code & Same functionality (forks, different language)                                  & 5 \\ \hline%\cline{2-3} 
UI            & Same steps to reproduce         & 2 \\ \hline
Permission          & \begin{tabular}[c]{@{}l@{}}Same configuration/environment\\(Permission set, Android/Window version)\end{tabular}  & 6 \\ \hline%5
Condition   & Same outcome (non-crashing)         & 35 \\ \hline%39
Stack trace & Same error/exception            & 39  \\ \hline %35
%Others      & Others                          &  \\ \hline
%Invalid     &                                 &  \\ \hline
\end{tabular}
}
\end{table}


==> study.tex <==
%\section{Motivation}
%Although Android apps are typically developed using Java programming language, they are different from traditional desktop applications and server applications. Particularly, Android applications rely heavily on a set of software components (e.g., Activity, Intent and Content Service Provider) supported by the Android Development framework with specific rules for managing these components~\footnote{http://developer.android.com/guide/}.
%
%%Crashes in Android applications arise due to several reasons, including (1) Android-specific bugs that occurs due to the complexity in Android activity lifecycle~\cite{hu2011automating,coelho2016exception}, and (2) programming mistakes that are also common sources of errors in Java development~\cite{coelho2016exception}. Meanwhile, prior work on automated testing and analysis~\cite{hu2011automating,coelho2016exception}
%%Despite the prevalence of crashes due to the complexity of Android activity lifecycle.
%
%Prior works on Android applications reveal that the complexity in Android activity lifecycle is one of the major causes of crashes in Android applications~\cite{hu2011automating,coelho2016exception}. Despite recent advances in automated testing and analysis of Android applications, there is no existing work that suggest patches to crashes in Android applications.

\section{A study of similar bugs in GitHub}
\label{sec:study-cause}
Given an open and unresolved GitHub issues $d$, identifying relevant GitHub issue $n$ that shares similar bugs with $d$ could be useful for localizing and fixing the bug in $n$. To design more effective tools to search for relevant GitHub issues, we need to first thoroughly understand the characteristics of similar bugs, including answering the research questions (\textbf{RQ1}-\textbf{RQ3}) listed in Section~\ref{sec:intro}. We investigate $RQ1$ because prior study shows that similar bugs could exist among two different applications~\cite{collabbug} but the characteristics of ``similar bugs'' have not been studied. We design $RQ2$ to investigate the usefulness of referring to GitHub issues with similar bugs. We study $RQ3$ to design better tools to better utilize information from GitHub issues with similar bugs. 

\input{study-table}

%\begin{description}[leftmargin=*]
%        \item[RQ1:] \emph{What are the common characteristics that define similar bugs?} What are the exact similarities in the related GitHub issues that developers refer to as ``similar bugs''?
%        %\item[Q2:] \emph{How often do developers refer to similar bugs in another repositories?} Specifically, what percentages of similar bugs are from two GitHub issues of different repositories?
%        \item[RQ2:] \emph{What strategies can we use to identify the pair of similar issues?} Can we derive a set of strategies to automatically identify these similar issues?
%        \item[RQ3:] \emph{How do developers make use of information about similar bugs?} Specifically, which software maintenance tasks that the similar bugs could assist developer with, if any? 
%\end{description}

%Same co(Android/Window version, Device, Permission set)

%We investigate $Q2$ to identify strategies that can be used to automatically search for issues with similar bugs. We study $Q2$ to investigate the prevalence of similar bugs found across different software project~\cite{collabbug}. 


To study the relationship between GitHub issues that share similar bugs, we manually inspected related GitHub issues. Our goal is to identify the information that we can obtain from GitHub issues with similar bugs. We first obtained a list of GitHub issues by searching for the keywords ``similar bug'' and ``similar problem'' for Java projects using \texttt{PyGitHub} (a Python library that interacts with GitHub API v3)~\footnote{https://github.com/PyGithub/PyGithub}. Our study focuses on Java projects because (1) most of the recent automated program repair techniques have been developed for fixing Java programs~\cite{xiong2017precise,jiang2018shaping,mei-et-al-ASE15,wen2018context,liu2019tbar} (including the recent bug report driven repair approach~\cite{bugreportrepair}), which indicates the importance of building an automated program repair system for Java programs; and (2) prior work on \cofind{} shows the existence of similar bugs across different Android apps while most Android apps are written in Java~\cite{collabbug}. For each issue $d$, our crawler searched for the first corresponding issue $n$ in which $d$ mentioned that $d$ and $n$ share similar bugs. The final output of our crawler is a list of GitHub issues ($d$, $n$) where $d$ and $n$ share similar bugs. Overall, our crawler searched through 4000 GitHub issues (GitHub API limits each search to 1000 search results~\footnote{https://docs.github.com/en/rest/reference/search}, so we search for the two keywords with 1000 open and 1000 closed issues separately), and identified 385 issues with links to similar bugs. From these 385 GitHub issues, we manually excluded 194 invalid issues (e.g., duplicated issues or irrelevant issues). After filtering the irrelevant issues, we identified \numstudy{} ($d$, $n$) pairs of GitHub issues where $n$ spans across \numstudyproj{} different Java projects. This relatively large number of open-source projects with GitHub issues mentioning similar bugs confirm our hypothesis that \emph{software developers tend to leverage the information about similar bugs during the discussion of a GitHub issue}.

 %We manually analyzed all issues and attempted to answer two questions:

% Overall, our crawler searched through 4000 GitHub issues (\texttt{PyGitHub} limits each search to 1000 search results, so we search for the two keywords with 1000 open and 1000 closed issues separately). From the original list of GitHub issues, we manually removed issues that do not have corresponding issues with similar bugs. After filtering the irrelevant issues, we identified \numstudy{} ($i$, $j$) pairs of GitHub issues that span across \numstudyproj{} different Java projects. %We manually analyzed all issues and attempted to answer two questions:

\subsection{RQ1: Characteristics of similar bugs}
For RQ1, we obtain the characteristic of similar bugs by reading carefully the GitHub issues, focusing particularly on comments made by developers when referring to the similar bugs (i.e., developers usually include explanation why the two bugs are similar). Then, we count the number of GitHub issues that exhibit the identified characteristics. 

The second column of Table~\ref{tab:study-tab} shows the common characteristics that define similar bugs in the evaluated pairs of GitHub issues, whereas the ``\# of Issues'' column denotes the number of GitHub issues that exhibit these characteristics. Our study shows that similar bugs can be defined by bugs that occur when two GitHub projects share the (1) same libraries, (2) same functionality, (3) same steps to reproduce, (4) same configuration/environment, (5) same outcome (exclude crash), or (6) same error/exception. As a pair of GitHub issues ($d$, $n$) can exhibit several similarities (e.g., they could share same libraries and produce the same error as the example in Table~\ref{tab:similar-bug}), we include all similarities in Table~\ref{tab:study-tab} (the category is mutually exclusive). Overall, our study shows that the most common characteristics of similar bugs are:
\begin{itemize}
\item Bugs that share the same library (76/\numstudy{} = 50\%)  
\item Bugs that share the same error/exception (39/\numstudy{} = 26\%)%26\%)
\item Bugs that share the same outcome (35/\numstudy{} = 23.33\%) %26\%)
\end{itemize}

The relatively high percentage of bugs that share the same library \emph{motivates the needs for automated dependency update tools}~\cite{dependabot,greenkeeper,macho2018automatically}.


 \begin{figure}
    \begin{minipage}[t]{\linewidth}
        \centering
        %\includegraphics[height=3.5cm,width=0.41\linewidth]{How_can_issues_help_4classes.png}
        \includegraphics[height=4cm]{fig/How_can_issues_help_4classes.pdf}
    \caption{The usefulness of similar bugs among 86 study issues}
    \label{fig:usefulness}
    \end{minipage}
\end{figure}

\subsection{RQ2: Usefulness of similar bugs}
\label{sec:usefulsim}
We investigate the usefulness of similar bugs by checking whether the \numstudy{} issues help developers to perform specific maintenance tasks by scoring them in the following order: (1) repair (most useful), (2) fault localization, (3) finding context of a bug, and (4) closing the issue faster (least useful). Specifically, if the similar bug could help developer directly in locating and fixing the bug, we select the most useful task (``repair'') rather than ``fault localization''. During our analysis, we exclude 64 GitHub issues from \numstudy{} because we could not determine their usefulness as there are no direct reply or discussion about the similar issue.

Given a pair of GitHub issues ($d$, $n$), we assess $n$'s usefulness based on the rationale explained below:
\begin{description}[leftmargin=*]
\item[Repair:] We consider $n$ as helping developer in $d$ to repair the bug in $d$ if: (1) the fix of $n$ could be directly applied to $d$, (2) the fix of $n$ only requires minor modifications before applying to $d$, or (3) the discussion of $d$ mentioned that they could find the fix for $d$ by referring to the information in $n$.
\item[Fault localization:] We consider $n$ as helping developer in $d$ to locate the bug if: (1) $n$ causes the bug in $d$, (2) $n$ includes fault localization information, or (3) the discussion of $d$ mentioned that they could identify the faulty location using the information in $n$. 
\item[Context:] We consider $n$ as helping developer in $d$ to finding more context for the bug in $d$ if the discussion in $d$ explicitly mentioned that they have learned something from $n$ (e.g., they gained some clues after reading $n$) but there is no further discussion about whether the knowledge gained had helped them in resolving the problem or identifying the fault. 
\item[Closing Issue faster:] We consider $n$ as helping developer in $d$ to closing the issue faster if: (1) after referring to the similar issue in $n$, the participants in the discussion of $d$ think that they cannot or do not need to fix the bug and decided to close the issue, or (2) $n$ only provides temporary workaround.
\end{description}

Figure~\ref{fig:usefulness} shows the usefulness of similar bugs among the 86 studied issues. Our study shows that similar bugs is most helpful in terms of helping developers to find more context (provide hints) for resolving the bug (\studycontext{} of studied GitHub issues). Meanwhile, \studyrepair{} of studied issues show the usefulness of similar bugs in helping developers to fix the bug. Overall, our results shows that \emph{similar bugs could help developers in resolving the GitHub issue in hand, especially in providing more context of the bug and fixing the bug}.

%situations of repair: 
%1. the fix of the referred issue totally applies to current issue
%2. the fix of the referred issue only requires minor modification to apply to current issue
%3. the participant found out fixes with the help of info in referred issues


%situations of fault localization: (however, if there is no further discussion about fix or workaround, we cannot decide if the participant identifies fault correctly, thus, in most times, I will classify them as context)
%1. the referred issue is the cause of current issue
%2. there is fault identification info in the referred issue
%3. the participant identified faults with the help of info in referred issues 

%situations of context:
%1. the author or other participants learned something from the referred issue, e.g., they had some clues, guess, or ideas inspired by the referred issue and explicitly state them as comments. However, no commends afterwards verify that the ideas successfully solve the problem or identify the fault. 

%situations of closing faster:
%1. after referring to the similar issue, participants think they cannot/don’t need to/ fix the bug and close the issue.
%2. the referred issue provides applicable temporary workaround


\subsection{RQ3: Strategies to identify similar bugs}
\label{subsec:rqtwo}
After identifying the common characteristics of similar bugs, we need to design strategies to automatically detect these characteristics. Specifically, as shown in Table~\ref{tab:study-tab}, we need to check if we can detect each of these characteristics from several available sources, including: (1) the description of a GitHub issue, and (2) information within different types of files that can be exploited for detecting these characteristics (e.g., Java projects typically has build files and Java class files, whereas Android project may have additional XML files for declaring app components and permissions). 

Given a pair of GitHub issues ($d$, $n$) that share a similar bug $b$, we derive \numop{} strategies to identify similar bugs based on the rules explained below:

\begin{description}[leftmargin=*]
\item[Dependency:] We check if $d$ and $n$ share the same libraries by comparing the set of dependencies shared by the GitHub issues in $d$ and $n$. For example, in Table~\ref{tab:similar-bug}, both \texttt{Maui} and \texttt{deeplearning4j} share similar dependency (\texttt{Stemmer}). Java dependencies are usually declared in build files. 
\item[Code:] We check if $d$ and $n$ share similar functionalities by comparing the Java code in the repository for $d$ and the code modifications in the patch mentioned in $n$. 
\item[UI (Android-specific):] We check if $d$ and $n$ share the same steps to reproduce the bug $b$ by comparing their interfaces that allow users to invoke these steps. In Android apps, interfaces refer to UI elements (e.g., buttons and text boxes) that are typically declared in XML files.
\item[Permission (Android-specific):] We check if $d$ and $n$ share similar environments by comparing the set of permissions that $d$ and $n$ acquire. We design this strategy as all Android apps need to declare the set of permissions in their manifest files but there is no such formal requirement for Java projects. The set of permissions is typically declared in XML files. 
\item[Condition:] We check if $d$ and $n$ share the same outcomes by comparing the conditions when the bug $b$ is triggered. This information is usually available in an issue's description.  
\item[Stack trace:] We check if $d$ and $n$ share the same error or exception by comparing their stack traces. For example, in Table~\ref{tab:similar-bug}, the issues in \texttt{Maui} and \texttt{deeplearning4j} share similar stack trace with similar exception. This information is usually available in the description of a GitHub issue.   
\end{description} 


 
%Table~\ref{tab:exception} shows the set of exceptions that lead to crashes in the investigated Android apps and the percentage of GitHub issues that arise due to particular exception. Table~\ref{tab:exception} illustrates that 
%The high percentage of \texttt{NullPointerException} confirms with the findings of prior study of Android apps~\cite{coelho2016exception}. 

%Note that the ``Unknown" row represents the scenario where the bug report did not include the information about the thrown exception. Although there are many such cases, this does not pose threat to our investigation as we could still derive the root cause of the crash through inspection of the bug-fixing commit.

%Table~\ref{tab:study-tab} shows the common root causes of crashes in Android apps we investigated. Column ``Category" in Table~\ref{tab:rootcause} describes the high-level causes of the crashes, while the ``Specific reasons" column gives the specific causes that lead to the crash. The last column (Category Total (\%)) presents the total percentage of issues that fits into a particular category. Overall, 14.02\% of crashes in our study occur due to the violation of management rules for Android Activity/Fragment lifecycles. The reader can refer to Section~\ref{sec:pattern} on the explanation of these lifecycle-related crashes. Meanwhile, 16.82\% of the investigated crashes are due to improper handling of resources, including resources either not available (Resource-related) or limited resources like memory (Resource limit). Furthermore, improper handling of callbacks contributes to 17.76\% of crashes. Note that this ``Callback" category denotes implementation-specific problems of different components in Android library (e.g., Activity, View and Intent). Among 40.19\% of NullPointerExceptions thrown in these crashing apps, only 12.15\% is related to missing the check for \texttt{null} objects (Missing Null-check). Interestingly, 4.67\% of the GitHub issues include comments by Android developers acknowledging the fact that the patch issued are merely temporary fixes (Workaround) for these crashes that may require future patches to completely resolve the crash.

%Overall, Table~\ref{tab:rootcause} shows that the complexity of activity/fragment lifecycle and incorrect resource handling are two general causes of crashes in Android apps. Moreover, ``Missing Null-check" in the ``Other" category also often leads to crashes in Android apps.



%Regardless what is the reason for introducing these errorsduring bug fixing and why they were not caught before re-lease, their common existences and severe impacts on users and vendors have raised some serious concerns about thebug fixing process. In order to come up with better process and more effective tools to address this problem, we need to first thoroughly understand the characteristics of incorrectfixes, including:

%We study $Q2$ because a survey of Android developers suggests that the topmost reasons (47\%) for \texttt{NullPointerException} in Android apps occur due to the complexity of activity/fragment lifecycle~\cite{coelho2016exception}. Our goal is to identify a set of generic transformations that are often used by Android developers in fixing Android apps. To gain deeper understanding of the root causes of each crash (Q1) and to identify the affect of activity/fragment lifecycle on the likelihood of introducing crashes (Q2), we manually examine lifecycle management rules in the official Android API documentations~\footnote{https://developer.android.com/guide/components/activities/activity-lifecycle.html}. 


%We focus on closed issues because those issues have been confirmed by the developers and are more likely to contain fixes for the crashes. From the list of closed issues on app crashes, we further extract issues that contain at least one corresponding commit associated with the crash. The final output of our crawler is a list of crashes-related closed issues that have been fixed by the developers. Overall, our crawler searches through 7691 GitHub closed issues where 1155 (15\%) of these issues are related to crashes. The relatively high percentage of crash-related issues indicates the prevalence of crashes in Android apps. Among these 1155 issues, 107 of these issues from 15 different apps have corresponding bug-fixing commits. We manually analyzed all issues and attempted to answer two questions:





%To study the root causes of crashes in Android apps, we manually inspect Android apps on GitHub and API documentation (as prior work has showed success in finding bugs via API documentation~\cite{Tan:2012:TTJ:2224481.2224930}). Our goal is to identify a set of common causes for Android crashes. We first obtain a set of popular Android apps by crawling GitHub and searching for the word ``android app'' written in Java using the GitHub API~\footnote{https://developer.github.com/v3/}. For each app repository, we search for closed issues (resolved bug report) with the word ``crash''. We focus on closed issues because those issues have been confirmed by the developers and are more likely to contain fixes for the crashes. From the list of closed issues on app crashes, we further extract issues that contain at least one corresponding commit associated with the crash. The final output of our crawler is a list of crashes-related closed issues that have been fixed by the developers. Overall, our crawler searches through 7691 GitHub closed issues where 1155 (15\%) of these issues are related to crashes. The relatively high percentage of crash-related issues indicates the prevalence of crashes in Android apps. Among these 1155 issues, 107 of these issues from 15 different apps have corresponding bug-fixing commits. We manually analyzed all issues and attempted to answer two questions:
%\begin{description}
%	\item[Q1:] What are the possible root causes and exceptions that lead to crashes in Android apps?
%        \item[Q2:] How does the complexity of activity/fragment lifecycle affect crashes in Android apps? 
%\end{description}

%We study $Q2$ because a survey of Android developers suggests that the topmost reasons (47\%) for \texttt{NullPointerException} in Android apps occur due to the complexity of activity/fragment lifecycle~\cite{coelho2016exception}. Our goal is to identify a set of generic transformations that are often used by Android developers in fixing Android apps. To gain deeper understanding of the root causes of each crash (Q1) and to identify the affect of activity/fragment lifecycle on the likelihood of introducing crashes (Q2), we manually examine lifecycle management rules in the official Android API documentations~\footnote{https://developer.android.com/guide/components/activities/activity-lifecycle.html}. 

%Indeed, the Android API documentation provides detailed explanations about the ``Lifecycle" and ``Resource" category, together with guidelines of the correct handling mechanism for these two categories.
%Therefore, we focus on the ``Lifecycle" category and the ``Resource" category for our derivation of program transformations.


==> syllabus.tex <==
\begin{table}[!t]
\caption{Weekly schedule and topics covered in the lab sessions}
  \label{tab:syllabus}
\begin{tabular}{r|l}
Week & Topics covered                                       \\\hline
1    & Roles in Software Development Teams     \\
2    & Git and GitHub                          \\
3    & GitHub Classroom and Markdown           \\
4    & Unit testing with JUnit                 \\
5  & Test coverage and Automated test generation with Evosuite                         \\
6    & PIT and Measuring Mutation Coverage     \\
7    & Metrics in Java Projects (MetricsReloaded Plugin)               \\
8    & Project planning        \\
9  & Static Analysis Tools (PMD, Checkstyle, and SpotBugs) \\
10 & Reverse Engineering and Testing Android Apps                                      \\
11   & Javadoc and Doxygen                     \\
12 & No class (Labor Week Holiday) \\
13  & Steps in Code Review  \\
14   & Progress Report Presentation  \\
15   & Common software vulnerabilities in Java programs \\
16   & Lab exercises for exam review                             \\
     &                                        
\end{tabular}
\end{table}


==> threat.tex <==
\section{Threats to validity}

\noindent\textbf{External.} Our study of similar bugs and our evaluation results may not generalize beyond the evaluated Java projects and Android apps. To mitigate this threat, we evaluate many open-source Java projects and Android apps that are popular in GitHub. Moreover, we perform our evaluation on open (unresolved) GitHub issues from real-world projects and made our data publicly available~\cite{our-web}.  

 %Furthermore, we also provide guidelines for students in their selection of the open-source apps to ensure the diversity of subjects in terms of popularity, ease of use, contains various test cases and a large number of reported GitHub issues. All participants of our study are fourth year CS students, and they are graded based on the number of new bugs discovered, which may lead to issues according to prior studies~\cite{carver2004issues,host2000using}. We countered this threat by using bonus points to increase student participation~\cite{ferrari2002using} and reward the same bonus points to students regardless of the testing approaches used in finding the new bugs. To counter the threat of the general applicability of our approach beyond the classroom setting, we found some examples where developers of Android apps referred to other related apps when filing a new bug report.
%could be demonstrated by the fact that in some selected issues, we observed that general app users may also refer to another related apps when filing a new bug report.

\noindent\textbf{Internal.} To reduce bias in selection of open issues, we wrote scripts to automatically crawl open GitHub issues from popular Java/Android projects. During the manual inspection and classification of the usefulness of each GitHub issue, two authors of the paper review the results independently and meet to resolve any disagreement.
% to reduce the influence on the results. %To avoid bias during the computation of the rank results for \mytool{}, we shuffled the rank results before presenting them to the two reviewers. 

\noindent\textbf{Construct.} Although many automated repair approaches are publicly available, we did not compare \mytool{} against them because to the best of our knowledge, \mytool{} is the first tool that uses the idea of \cofix{} for debugging and program repair. Moreover, we evaluate the effectiveness of \mytool{} mainly based on the relevance and the usefulness of the recommended GitHub issues but other aspects (e.g., the time taken in reading and understanding the recommended issues) could be important. We mitigate this threat by reporting all issues that we considered useful to developers, and manually analyzing developers' feedback.

